Shenjing: A low power reconfigurable neuromorphic accelerator with partial-sum and spike networks-on-chip

The next wave of on-device AI will likely require energy-efficient deep neural networks. Brain-inspired spiking neural networks (SNN) has been identified to be a promising candidate. Doing away with the need for multipliers significantly reduces energy. For on-device applications, besides computation, communication also incurs a significant amount of energy and time. In this paper, we propose Shenjing, a configurable SNN architecture which fully exposes all on-chip communications to software, enabling software mapping of SNN models with high accuracy at low power. Unlike prior SNN architectures like TrueNorth, Shenjing does not require any model modification and retraining for the mapping. We show that conventional artificial neural networks (ANN) such as multilayer perceptron, convolutional neural networks, as well as the latest residual neural networks can be mapped successfully onto Shenjing, realizing ANNs with SNN's energy efficiency. For the MNIST inference problem using a multilayer perceptron, we were able to achieve an accuracy of 96% while consuming just 1.26mW using 10 Shenjing cores.

==> Arxiv-Shenjing with app/architecture.tex <==
\label{sec:arch}

%{\bf Peh: Can MNIST's full network 28-784-512-10 be drawn as overlay on top of 4x3 tiles, replacing or extending Fig 1(a)? And remove Unused cores in legend.}

\begin{figure}[t]
\includegraphics[width=0.9\linewidth]{Figures/4X3Overview.pdf}
\caption{Mapping of MNIST-MLP onto Shenjing.}
\label{fig:neuron_core_abstract}
\end{figure}

\section{Architectural overview}
\label{sec:architecture}

In a SNN, two key operations are performed at each layer of neurons: (1) weights of incoming synapses that spiked are summed, and (2) if this sum exceeds a threshold, a spike is sent to the next layer.
%Shenjing is a SNN hardware accelerator architected specifically to support these operations, the summation of weights, and communication of spikes, in a configurable fabric, thus enabling transfer learning of ANN models. This section describes Shenjing's architecture while the next section dives into the toolchain that automatically maps ANN models onto Shenjing's SNN accelerator.
Figure~\ref{fig:neuron_core_abstract} illustrates a Shenjing chip with 10 cores arranged in a grid where each core has 256 neurons interconnected by per-neuron NoCs that are meshes. 
Weight summation, is handled first by the neuron core and then via the 256 {\it partial sum NoCs} (PS NoCs) that perform in-network additions across cores. %Partial sum NoCs have adders embedded within the routers, so partial sums are accumulated among the cores as they are routed.
Spiking is handled by the 256 {\it spike NoCs} that generate and communicate 1-bit spikes across cores. 

Shenjing's NoCs are software-defined, having the twin benefits of reconfigurability and low hardware overhead. The software mapping tool (see Section~\ref{sec:map}) maps neurons to cores, sets up the adder tree topology, configures the PS NoCs, and connects up the cores with the spike NoCs. The per-neuron NoCs enable simple mapping of neural network models onto Shenjing. 
Software-defined configurations are stored in Shenjing's configuration memories, governing the cycle-by-cycle operation of the hardware. The NoC routers are thus freed from handling any run-time routing or flow control, significantly simplifying their design. 

Figure~\ref{fig:neuron_core_abstract} shows a simple mapping of a fully connected network for MNIST as Table~\ref{table:applications}(a) on Shenjing. 
As each core only holds 256 neurons, the 784 MNIST inputs can be evenly mapped onto 4 cores and the hidden layer of 512 neurons can be mapped onto 2 cores. The spikes from the input layer to the first half of the 512 neurons are mapped onto cores (3,0), (2,0), (1,0) and (0,0). Similarly, the spikes to the other 256 neurons are duplicated and mapped onto cores (3,1), (2,1), (1,1) and (0,1). The output layer fits onto cores (0,2) and (1,2).

\begin{comment}
In the first phase, neuron weights are stored in the cores' SRAMs, and fed to accumulators that do a weighted sum across all neurons in the core. Each neuron core is configured as 2x2 subcores so as to double the SRAM operating frequency and corresponding performance of weighted sum. Unmapped subcores and SRAM lines are gated for power saving (see Section 3.2). Note that the MNIST example has no unused subcores.
\end{comment}
First, weighted sum is performed within each neuron core to form the local partial sums. Next, the corresponding local partial sums (PS) from (3,0) and (3,1) are injected into the partial-sum NoCs, to cores (2,0), (2,1) which adds them with their local core's sum, respectively. Cores (1,0) and (1,1) proceed similarly. Finally, at cores (0,0) and (0,1), the PS accumulates with those from cores (2,0) and (2,1) to create the full weighted sum which is fed to the spike generation unit at cores (0,0) and (0,1) to determine if a spike should be fired. 

%As the aggregation direction in Figure~\ref{fig:neuron_core_abstract}(c) illustrates, at first all PS propagate from low-level leaf nodes to the middle-level leaf nodes (0,0), (0,1), (2,0), (2,1) and then arrive at root nodes (0,0) and (0,1) to complete the hidden layer. At the output of FC1, spikes are generated when the accumulated PS exceeds the threshold. Spikes are then routed to the next layer of the SNN, mapped to cores (0,2) and (1,2) via spike NoCs, triggering a similar in-network PS calculation tree that ends at root node (0,2). At (0,2), the final sum feeds the spike unit and determines the final output. 


\begin{figure*}[bth]
\centering
\includegraphics[width=0.9\linewidth]{Figures/core_ps_spike.pdf}
\caption{Micro architecture of (a) a neuron core (b) a partial sum router and (c) a spike router.}
\label{fig:core_ps_spike}
\end{figure*}

%Peh: Sep 2: Up to here... will work on the rest of Section 3 later today
Figure~\ref{fig:core_ps_spike} details the microarchitecture of Shenjing's neuron core, partial-sum and spike routers.

\noindent{\bf Neuron core.}
\label{sec:arch_neuron_core}
Each neuron core is a collection of weight synapses stored in 4 SRAM banks, computing elements (neurons) implemented with accumulators, and control logic~\cite{truenorth}~\cite{Merolla2014TrueNorth}.
 
%A neuron operation starts by receiving concurrent axon values from the input interface, then accessing synaptic weights in memory row by row. The weights, which are learnt earlier during training, are stored in SRAMs in column-wise fashion, with respect to a neuron. When an axon is `1', the SRAM is read for its corresponding weight to form a synaptic connection. When it is `0', the read operation will be skipped. Every time the data is read out from an SRAM column, it is fed to an accumulator and then registered to complete a weighted sum. This in-memory processing is also found in other SNN implementations

%{\color{blue}
%Could the authors provide experiments to show how the introduction of banking and power gating are beneficial in different applications? Does power gating at the bank level have any significant effects?
%}

%The full neuron core is decomposed to 4 sub-cores internally, where each subcore has 128 axon inputs and 128 neurons as Figure~\ref{fig:core_ps_spike} (a) depicts. This configuration has two advantages. Firstly, when SRAM bank1/bank2 and bank3/bank4 work in parallel to process 256 inputs, the pipeline latency is reduced from 256 consecutive reads to 128, doubling performance viz-a-viz a single 256-input SRAM. Secondly, if fewer neurons are needed, as is the case in our MNIST example where only 10 neurons are required for the FC2 layer, bank3 and bank4 will be gated. This will save 50\% of leakage power from SRAMs and 50\% of active power in a neuron core. In other applications, total power can be saved as much as 75\% when the mapping algorithm trades-off core utilization with routing/locality. Section 5 will demonstrate the performance improvement and area tradeoff of this neuron subcore microarchitecture in detail through RTL synthesis. 

%We continue the MNIST example to illustrate how a bank in the neuron core works (Figure~\ref{fig:core_ps_spike}(a)). Initially bank2 at core (3,0) receives 128 input spikes \textit{b(t)} at \textit{t=1}, specifically, $b_{1}$ = $b_{2}$ = $b_{3}$ = $b_{4}$ = `1' and $b_{5}$ = `0'. The corresponding cached weights of $w_{1}$ to $w_{5}$ along the bitline are {\tt 11001}, {\tt 00110}, {\tt 11101}, {\tt 00010} and {\tt 00110} respectively. Next the SRAM bank triggers reading of the weights one by one till $b_{5}$ disables the read of $w_{5}$ as their weighted sum will be zero irrespective of the weight. The neuron accumulates the readout weights simultaneously and converts the accumulated value after each read to 2's complement to form a 13-bit weighted sum of {\tt 1111111111110}. The sum is then stored in a register, completing the single neuron's operation.

%After 128 weighted sums are sampled from their registers, they are summed up and combined with the sums from the other banks in the `Combine and MUX logic' to form 256 partial sums of the entire neuron core which are each injected into the corresponding 256 partial-sum routers to compute the full weighted sums within the PS NoCs.



%Peh: Will move accuracy discussion later on.
%Previous neuromorphic architectures, including TrueNorth, \cite{truenorth}~\cite{Merolla2014TrueNorth} do not explicitly support partial sums across cores.When a layer cannot fit within a core, each core accumulates based on a subset of axons and synapses, which formulates a partial sum, then integrates and fires a spike accordingly. An aggregating core sums these spikes to gain a representation of full weighted-sum and generates a final output for the layer. As explained in Section 2, this work-around method leads to accuracy loss that worsens with deeper networks. 
%Unlike conventional SNN architectures where cores only output spikes, Shenjing's cores can output weighted sums as well into the partial-sum NoCs which perform full accumulation of the partial sums at the routers, along the way from source neuron core to the destination core. In these networks, adders are embedded within the routers which are connected to each neuron core, and each partial sum router can be configured to add sums coming in from any input port, or a previous result stored in the router, scheduled by the mapping tool (see Section 4).
%Shenjing comprises 256 partial-sum NoCs, in a mesh topology, each assigned to a single neuron within the neuron core. 

\noindent{\bf Partial Sum NoCs.}
A $4 \times 2$ input crossbar fetches input data from a port (North, South, East or West) and either registers it for local addition or bypasses this router to adjacent routers via output links. The $3 \times 5$ output crossbar ejects it to the desired port or the spiking logic of the neuron core. Our mapping software constructs a PS adder tree by configuring the crossbars of the PS NoC router appropriately. These configuration bits are loaded into a configuration memory prior to Shenjing execution, and drives the select signals of the crossbars and muxes. Each PS NoC is dedicated exclusively to the same neuron in each core, and the software mapping tool maps neurons appropriately (see Section~\ref{sec:map}). Hence, unlike conventional NoCs, the PS NoC does not need buffer queues, flow control or routing logic.

PS NoCs' bitwidth corresponds to the data width of the synaptic weight and adders within the routers. When two $n$-bit numbers are added, the sum is $n+1$ bits. Having a 16 bit width allows us to sum up $2^{11}$ 5-bit weights at the worse case where all weights are {\tt 11111} with all input spikes being `1'. In practice, the sparsity of spikes allows even more accumulations. 
We did not encounter any overflow in our applications. 

%Continuing with the MNIST example, core (0,0) first adds up partial sum from core (1,0) with its own local partial sum. The input is registered at south port and the crossbar connects the south register to path OP2 while the local partial sum is multiplexed into OP1. The adder then sums the incoming data from OP1 and OP2. Similarly, the sum is added up with another partial sum from core (2,0) which is ejected from the north port of its partial sum NoCs. When the summation is completed, the output crossbar sends the full weighted-sum to the spiking unit in the core. 

\noindent{\bf Spike NoCs.} A multiplexer selects either the local partial sum from the neuron core (when a layer fits entirely in a core), or the full weighted-sum arriving from the PS router (when a layer spans multiple cores) as input for the spiking logic unit. The latter integrates the sum and compares the potential against the threshold. If it exceeds the threshold, a spike is generated, and the potential value is subtracted from the threshold. The 1-bit spike then enters the $5 \times 5$ crossbar where it is buffered and sent to the next hop in the spike NoC. %Every neuron has a spike NoC which is 1-bit wide, and completely software-scheduled -- the configuration memory dictates the port connections of each spike NoC crossbar every cycle. 

%In the MNIST MLP example, the full weighted-sum is computed at the partial sum router of core (0,0), and passed to its spike router. A spike is generated by the spiking logic which the spike router routes to the East output port, as directed by the \textit{in\_sel, out\_sel} signals in the configuration memory. The spike next arrives at intermediate core (0,1)'s spike router, traverses the crossbar from the west to east port, towards (0,2). When it finally arrives at destination core (0,2), the spike crossbar is made to connect the west input port to the eject port that connects to the neuron core as axon input.

Shenjing's spike NoCs support hardware multicast. A single spike packet injected by a neuron core can be scheduled by software to be X-Y routed to successive multicast destinations, ejecting the spike when it arrives at each destination in turn. 
%Compared to multiple unicasts, this reduces traffic load substantially, and is readily supported in the spike NoC router circuit because the crossbar can support an incoming port connected to multiple outgoing ports. 
Hardware multicast is particularly useful when mapping CNNs onto Shenjing, when spikes from a core are often sent to multiple cores located next to each other. 

%{\bf Peh: Huh? But the hardware can support simultaneous multicast (1-to-many) and aggregation (many-to-1) at a single router -- Why sequentially?? Can u illustrate one multicast example using the MNIST in Fig 1 and 3?}
 
\noindent{\bf Reconfigurability and accuracy.} %Shenjing's per-neuron PS and spike NoCs are designed to achieve its primary goal of transfer learning, to allow software to freely map neurons onto neuron cores, so myriad neural network models can be naturally overlaid onto the hardware. 
Prior SNN accelerators~\cite{Merolla2014TrueNorth, spinnaker,shi2015development} chose block-level spike connectivity instead, so an entire block of multiple spikes is routed together to the same destination block. Block-level spike NoCs amortize the hardware cost of dynamic routing and flow control across many spikes. Shenjing is able to support neuron-level bit-wise spike NoCs because our spike NoCs are completely software-defined, so such hardware overheads are not an issue. As most ANNs demand arbitrary connections to cores at diverse locations, Shenjing's per-neuron NoCs provide the most flexible substrate for configuring ANNs onto our SNN hardware.

Previous SNN architectures communicate strictly using spikes across cores, and do not support partial sums. When a layer cannot fit within a core, each core computes a partial sum based on the subset of axons and synapses within the core, then integrate and fire a spike. An aggregating core sums these spikes to gain a representation of full weighted-sum and generates a final output for the layer. This can lead to significant accuracy loss. Prior SNN architectures side-step this by requiring SNN models to be developed and trained from scratch, taking into account hardware core size constraints (see Section~\ref{sec:related-works}). Shenjing eliminates such accuracy loss with its PS NoCs that precisely add weights between cores within the network, thereby allowing software to easily map pre-trained models onto Shenjing hardware.




==> Arxiv-Shenjing with app/background.tex <==

\begin{comment}

\subsection{Conventional artificial neural networks}
We shall now give a brief introduction into ANNs and their common layer structures. An artificial neuron $i$ will perform weighted sum across all its inputs and apply an activation function to produce the output to the next layer:
\[
y_i=f(\Sigma_{j=1}^n (x_j\cdot w_{j,i})).
\]

{\bf Fully Connected Layer.}
In a fully connected layer~\cite{taylor1996neural}, each neuron receives all inputs from the previous layer to produce the output.

{\bf Convolution Layer.}
In a convolution layer~\cite{lecun1995convolutional}, a kernel sweeps over the input spatial dimensions and perform the weighted sum to produce the output.

{\bf Pooling Layer.}
The pooling layer is a sub-sampling layer that reduces the size of the inputs by taking average, max, etc. operations among the inputs in a kernel.

{\bf Residual Network.}
As the state-of-the-art network structure in deep neural networks, residual networks~\cite{he2016deep} allows a layer's output to be duplicated, with one set going on the usual route, and the other rerouted and added directly to a much later layer.
\end{comment}

\subsection{Spiking neural networks}
SNNs~\cite{maass1997networks} are considered third-generation neural networks. Comparing to ANNs, where the inputs and outputs are real values, SNNs work with input/output of streams of binary values along the time dimension called {\em spike trains}. In this work, we use the integrate-and-fire (IF) model. For each neuron, there are two major steps in the IF model:
\begin{enumerate}
\item {\bf Integration.} The {\em membrane voltage} of the $i$-th neuron at $t$-th time step is the integration of the weighted sum of its binary inputs $b_j(t)$ at $t$ and its value at previous time step $(t-1)$.
\begin{equation*}
V_i(t)=V_i(t-1)+\Sigma_{j=1}^{n}(b_j(t)\cdot w_{j,i}).
\label{eq:integrate}
\end{equation*}

\item {\bf Fire.} If the membrane voltage exceeds a preset threshold, $\theta$, the neuron {\em spikes}, i.e., outputs `1', and the membrane voltage is decreased by the threshold. Otherwise, the neuron outputs `0'. In other words,
if $V_i(t) \geq \theta$ then $y_i(t)=1$, and $V_i(t) = V_i(t)-\theta$. Otherwise, $y_i(t)=0$.

\end{enumerate}

SNN uses the similar network structure and feed-forward inference as ANN, such as multilayer perceptron (MLP) and convolutional neural network (CNN). In this paper, we present both MLP and CNN applications.


\subsection{SNN traits} {\bf Peh: Weaving this into intro}
Compared with ANNs, SNNs are more energy efficient. First, data passing through the layers are binary, so the computation of weighted sum is performed by addition instead of multiplication. This reduces computation power and time significantly. Moreover, a SNN will perform an addition only when the input is $1$, whereas ANN performs multiplications on all neurons across all inputs. In practice, the spiking of neurons is usually sparse, thereby substantially reducing the number of additions.

Using binary instead of full precision floating point data brings about a loss in accuracy. This is the main disadvantage of SNN. However, for most applications, the amount of accuracy loss is usually acceptable. As a matter of fact, there are many researchers working on the compression of ANN by reducing the precision of weights, activations or gradients at the cost of accuracy loss~\cite{han2015deep,zhou2016dorefa,courbariaux2016binarized}.

\subsection{From ANNs to SNNs}
\label{sec:need-PS-Noc}
Due to the discontinuity in the formulation of SNN making the functions to be learnt non-differentiable, there is no robust supervised learning algorithm that is analogous to back-propagation for ANN. Instead, a SNN is usually converted from a pre-trained ANN using the same neural network structure, but with the equivalent ANN's continuous activation replaced by {\em spiking rate encoding}~\cite{Diehll2015}. The input is first converted to a {\em spike train} of a pre-defined length $T$ that has the corresponding normalized value as the spiking rate. Weights of each layer are then normalized such that the spiking rate of each layer correctly represents the ANN activation. 
As an example, suppose we have an ANN whose input is a greyscale picture with pixels of value in $[0, 255]$. Since the equivalent SNN can only take binary inputs of spikes (i.e., 0's and 1's), we need to encode the input. So, the input is first normalized to $[0,1]$ by dividing each pixel value by 255. We then generate a random sequence of spikes (the spike train) of length $T$ as follows: for a pixel value $x\in [0,1]$, we will randomly generate a sequence of about $xT$ ones and $(1-x)T$ zeros. For instance, a black pixel which is 255 will be converted into a $T$-bit spike train of all ones. This spike train is then fed to the neurons in input layer, one spike at a time, across $T$ time steps. Next, for each layer we use the trained ANN weight normalized by the maximum of activation values to ensure that each neuron spikes at most once in a time step. At the output layer, the neuron with the highest number of spikes in $T$ steps is taken as the prediction. 
It has been shown that such a conversion will result in a small accuracy loss~\cite{rueckauer2016theory}. %For not too large networks, the relative loss in this loss is typically less than 5\%. 
In Table~\ref{table:benchmark}, the ``abstract SNN accuracy'' shows the accuracy of our applications converted from ANN to SNN, before mapping onto hardware architectures. Accuracy degrades just 3-6\%.
{\bf Peh: Mentioning key point above in intro to argue that accuracy of SNN models is ok -- need one more huge network}

\begin{comment}
{\bf Peh: Can you add a table showing various ANN network models and their resulting SNN network model accuracy, when everything is run in *software*, regardless of hardware core constraints? Showing that the accuracy loss is very small? So that later we can also highlight how Table 6's Shenjing's accuracy is the same as the SNN software model accuracy. I think we also need a figure or example walking through how this ANN to SNN model conversion is done, or at least how you manually did it for the various models we used in this paper.}
\end{comment}



\subsection{\color{red}Overcoming the partial sum problem}
\label{sec:SNN-to-hw}
{\bf Peh: I think this should be weaved into Architecture of PS NoCs explaining how configurable PS NoCs help with accuracy too, in addition to energy and configuration.}
There is however a second source of accuracy loss. Existing SNN hardware such as TrueNorth~\cite{truenorth} are organized into cores due to hardware constraints as well as for better utilization. Each core computes the weighted sum addition of neurons followed by spike generation.
 Cores communicate strictly using spikes. This presents an issue when layers are too big to fit onto a single core and has to be split. {\color{red} {\em spike}() is a binary function that returns a `1' if its argument exceeds a threshold and `0' otherwise. It is applied to the sum of weights. If we break the sum of (signed) weights into partial sums, i.e. $W = W_1 + \cdots + W_n$, then, as far as we know, there is no function, $\odot$, that will guarantee that
 $spike(W) = spike(W_0) \odot \cdots \odot spike(W_n)$. Systems like TrueNorth
introduce a new layer to combine the spikes from the split layers. 
However, the information loss causes further accuracy loss because depending on the values of the activated weights cancels out each other, spurious spike may sometimes be generated, and this cannot be eliminated entirely by learning in the new layer.} 
\begin{comment}
Consider this simplified extreme: suppose we have a sequence of positive and negative numbers (weights) to be summed. Now suppose that the numbers cancel out and the sum is zero - hence no spike. If we split this into two separate sums, it could be that we ended up with the positive numbers all end up in one sum, and the negative in the other. The net result is that in one core, a spurious spike would be triggered and propagated to the combination layer.
\end{comment}
 
{\color{red}Shenjing eliminates such accuracy loss with its partial sum NoC, which receives the weighted sum of the cores and adds them up precisely. In the above example, Shenjing can produce the total weighted sum over all 784 inputs and produce spikes based on the total sun. This also removes the need for the new combining layer.}

To see the impact of splitting up a layer, we tested a brute-force implementation~\cite{lee2019system} of the MNIST-MLP application (see Table~\ref{table:applications}) for a TrueNorth-like architecture (with no partial sum NoC). %The results are shown in Table~\ref{table:applications}. 
According to their algorithm, in the first layer, when the MNIST input size 784 is larger than a 256-neuron core size, the inputs are split onto 4 cores, and as the layer output size is 512, we need two groups of them with duplicated input. In each group, a core receives 196 input spikes, performs the weighted sum, and spikes with 1/4 of the original threshold. The spikes from 4 cores are then merged by 2 additional cores to produce the final output of the layer. The same method is applied to the second layer. In the end, the method uses 5 additional cores to merge spikes. With 256-neuron cores, we saw MNIST-MLP's accuracy drop from 96.11\% in Table~\ref{table:benchmark} to 93.61\%. The more splits (due to larger models that have to straddle multiple hardware cores), the higher the accuracy loss. To illustrate this, we use the same splitting approach above to map MNIST-MLP onto a range of core sizes. As core size reduces to 128 and 64, thus forcing more splits, we saw the accuracy dropping further to 92.69\% and 88.09\%, respectively. On the other hand, Shenjing maintains the original 96.11\% accuracy of the abstract SNN model.




==> Arxiv-Shenjing with app/conclusion.tex <==
In this paper we introduced Shenjing, a SRAM-based SNN accelerator for on-device AI. Unlike previous works on SNNs that attempt to mimic the brain, Shenjing has a more practical goal of providing an architectural means to map trained ANNs onto energy-efficient SNNs. The key to enable such transfer learning in a scalable way lies in the software-defined partial sum NoCs and per-neuron spike NoCs. This paper also outlined the mapping algorithm that will exploit these NoCs efficiently when mapping ANNs into SNNs. Our results show that on a 28nm technology node, Shenjing is able to implement the CIFAR-10 ResNet deep learning benchmark using 5863 cores and  0.887W while achieving 72.50\% accuracy. 

==> Arxiv-Shenjing with app/discussion.tex <==
{\bf Core reuse.}
%As CNNs grow deeper, one can always find a network exceeding the hardware limit if all layers are flattened on the cores. Therefore, it is important for a neuromorphic hardware to support core reusing, meaning one hardware core can be used as multiple logic cores. 
Shenjing can easily support a type of core reuse without reloading the weights. In our current mapping of a convolution layer, the input channels are mapped to multiple cores. All channels use identical weights and operations along the spatial dimensions and add up their weighted sums. So, we can use just one core to process all input channels and add them up within the core. The hardware needs to support accumulation of multiple weighted sums from the neuron core, but that cost is small. A more general core reuse strategy where the weights are swapped out and reloaded will have a much higher overhead.

%In principle, core reuse transfers the cost in area to time, thus impacting throughput. For embedded and real-time systems that neuromorphic hardware targets, trading off throughput for area is an important design decision.
%Throughput is important for neuromorphic hardware because they target embedded and real-time systems. Therefore, whether to support core reuse, and what level should the reuse be at is a design choice for architecture developers.

{\bf Mapping optimization.} We used a simple greedy mapping algorithm for our current workflow. This mapping is essentially the well-studied static task graph mapping on multiprocessor problem~\cite{mapping}. We will consider using other more refined algorithms in our future work.

%{\bf Weight Precision.}
%\label{sec:discuss-precision}

%{\bf NoC topology.}
%We chose simple meshes for all our NoCs for several reasons: It provides a universal fabric for software configuration, easing mapping. A lower degree topology like rings will lead to lower power overheads, but heavily constrain the software mapping tool. As our NoCs rely on software for routing and flow control, hardware cost is low anyway. 
%As for hierarchical or clustered topologies, ANNs connections tend to be between layers of many neurons, so there is little locality within a layer that a clustered topology can benefit from. Besides, SNNs are not latency sensitive, so the high average hop count of meshes when compared to hierarchical topologies has little effect on benchmark performance. %{\bf Peh: True and demonstrated in Section 6? If instead of a mesh you have say 16 tiles connected to one router, so fatter routers but fewer hops, will that help?}. 
%Meshes also lend themselves readily to hardware floorplanning and full-chip place-and-route, simplifying fabrication.

%{\bf Multiple chips.}
%Number of IOs across chip, bandwidth, our fully distributed architecture inherently lends itself to multichip.
%Cite current pin bandwidth, serial IO bandwidth to back our assumptions in Section 7 results.
%Peh: I think the above will already be mentioned in results

%{\bf SRAMs with synthesized accumulators for memories.} State-of-the-art neuromorphic architectures have started using non-volatile memory for better energy efficiency~\cite{Jo2010Memristor}~\cite{Ambrogio2016RRAM}~\cite{Wang20152T1R}. For instance, resistive switching memory (RRAM) device has advantages of density, parallel synaptic operations, etc. However, RRAM is still an immature technology that needs much improvement to enable multilevel operation, high on/off ratio, and linear change of the resistance~\cite{Daniele2018NVM}. Shenjing's architecture is orthogonal to the memory technology; we utilize memory compiled SRAMs on the 28nm commercial process, designing the rest of Shenjing around that. The accumulators within our neuron core are synthesized logic, leading to 128 13-bit adders synthesized for each sub core, and (128*4+256=768) 13-bit adders. This is why our neuron core (SRAM+accumulators) takes up 97.6\% of total Shenjing power for the MNIST MLP application. This can be optimized by custom designing in-memory compute SRAMS, like TrueNorth, similar to~\cite{VermaJSSC2017}, which will dramatically reduce the neuron core power and energy. 
% and can be readily optimized just by scaling down the supply voltage. In addition, low power SRAM techniques such as ~\cite{Clinton2017SRAM}~\cite{Guo2018SRAM}~\cite{Chang2017SRAM} can deliver substantial power and energy savings. 

{
%\color{red}
{\bf Optimization of neural network models.}
In ANN, many optimization techniques have been proposed. Some of these such as pruning connections~\cite{han2015deep}, and quantization to weight and gradient~\cite{zhou2016dorefa} are compatible with SNN models, and thus with Shenjing. However, as the activation of SNN is binary, there is little room for further compression. Binarized Neural Network (BNN)~\cite{courbariaux2016binarized} can be considered as a special case of SNN, and Shenjing can support BNN with minimal modification. \cite{ji2018bridge} proposed a compiler to map SNN to hardware architectures by first allocating the network to cores before tuning the weights. Their core allocation algorithms can be used on Shenjing, but the need for weight tuning is eliminated with Shenjing's partial-sum NoCs.

}


{
\color{red}
{\bf Scalability of Shenjing}
SNNs target resource constrained user-cases. Most state-of-the-art SNN accelerators~\cite{Esser11441, spinnaker, inxs} including TrueNorth limit their applications to $32\times 32$ RGB images like Cifar-10, and their models to convolutional networks. Shenjing has a similar target, and we have demonstrated its applications with up to 5863 cores. Thanks to its NoC, it is also the first SNN architecture to support ResNet.}


==> Arxiv-Shenjing with app/intro.tex <==
The phenomenal success of deep learning has led to the use of specialized hardware accelerators such as Google's TPU in data centers, driving cloud-based AI. On-device AI will be next: Applications with stringent timing, form-factor, energy, privacy requirements will demand AI on embedded devices. Compared with ANNs, SNNs are inherently more energy-efficient. First, data passing through the layers are binary, so computation of weighted sum is done through additions, instead of multiplications. This reduces computation power and time significantly. Moreover, a SNN will perform an addition only when the input is $1$, which in practice is very sparse, whereas ANN performs multiplications on all neurons across all inputs. While the compute requirement is ameliorated, the on-chip movement of data, i.e., communication, now dominates cost. %Optimizing communications is thus the main focus of this work.

We propose Shenjing, a reconfigurable SNN accelerator, whose essence lies in its per-neuron software-defined on-chip networks (NoCs) that allow software to configure and link up individual hardware neurons to match myriad neural networks. Summation of weights is efficiently performed enroute within Shenjing's partial sum NoCs, followed by the generation of spikes which are configured to route each neuron to its next layer neuron through Shenjing's spike NoCs. By exposing all on-chip communications to software configuration, 
Shenjing's NoCs can be ultra-lightweight, requiring no buffer queues or virtual channels and no routing or flow control logic. 

Shenjing's software-defined NoCs also enable run-time reconfiguration. While energy-efficient SNNs are particularly suited for on-device AI, they are not currently widely used. Deploying SNNs will require the development and training of new models from scratch, a major hurdle to deployment. Shenjing's reconfigurability allows for the mapping and transfer learning of widely used ANNs onto Shenjing's SNN hardware, bootstrapping SNN deployment.

\begin{comment}
The contributions of this work can be summarized as follows:

\begin{enumerate}
\setlength{\itemsep}{0pt}
\item Our architecture is completely software-scheduled, and thus requires just lightweight hardware. A 28nm 2cm$^2$  Shenjing chip that houses 784 cores or the equivalent of 51,380,224 synapses (realized by 256 28x28 partial sum mesh NoCs and 256 28x28 spike NoCs) consumes about 100~mW.
\item We present a corresponding transfer learning based configuration toolchain that maps existing ANN deep learning models, from fully connected to convolutional, pooling layers, and for the first time residual networks, onto our SNN-based hardware.
\end{enumerate} 
\end{comment}

% Section~\ref{sec:architecture} describes the overall architecture of Shenjing, with its software mapping tool detailed in Section~\ref{sec:map}. Our evaluation results are discussed in two sections. Section~\ref{sec:synthesis} provides the RTL circuit level results while Section~\ref{sec:sys} presents the end-to-end application level results. This is followed by a brief survey of the vast literature of related works in Section~\ref{sec:related-works}, and the conclusion.


==> Arxiv-Shenjing with app/mapping.tex <==
%Peh: Will need to explain transfer learning: how learned weights are converted to spikes. Cos background section removed

Figure~\ref{fig:compiler_overview} shows our
toolchain that automatically maps a trained SNN onto Shenjing. In the first logical mapping phase, the toolchain maps each layer's weights onto a set of logical cores, and then schedule the logical PS NoCs to produce the total weighted sum within the layer. It also schedules the logical spike NoCs to direct the spikes among layers. In this phase, NoC scheduling determines just the source and destination. Next, in the physical mapping phase, logical cores are placed onto physical chips, and the logical NoC scheduling is implemented as cycle-by-cycle routing instructions.

\begin{figure}[ht]
\includegraphics[width=0.8\linewidth]{Figures/compiler_overview.pdf}
\caption{Shenjing's software mapping tool flow.}
\label{fig:compiler_overview}
\end{figure}

%\subsection{Logical Mapping}
\noindent{\bf Logical core and partial-sum NoC mapping.}
When the number of inputs to a layer exceeds the size of a core, we split them into multiple cores, and accumulate the partial weighted sum using the partial-sum NoC. %Here, we explain the mapping algorithms for fully connected and convolution layers.

1. {\em Mapping fully connected layers}:
To map an $m\times n$ fully connected layer with $m$ inputs and $n$ outputs where both $m$ and $n$ exceed the core size, we need $n_{\mbox{\scriptsize row}} \times n_{\mbox{\scriptsize col}}$ cores, where $n_{\mbox{\scriptsize row}}=\lceil m/N_{\mbox{\scriptsize in}}\rceil$, $n_{\mbox{\scriptsize col}} = \lceil n/N_{\mbox{\scriptsize out}}\rceil$ and $N_{\mbox{\scriptsize in}}$ and $N_{\mbox{\scriptsize out}}$ are the number of synapses and neurons of one core. We arrange the $n_{\mbox{\scriptsize row}} \times n_{\mbox{\scriptsize col}}$ cores in a rectangle. The rows receive the $m$ inputs and columns produce $n$ outputs.
Algorithm~\ref{alg:scheduleFC} shows the logical scheduling of partial-sum NoCs to produce the total weighted sum.
\begin{algorithm}[ht]
\footnotesize
  \caption{Software mapping algorithm for a fully connected layer onto Shenjing's partial sum NoCs. }    \label{alg:scheduleFC}
  \SetKwInOut{Input}{Input}
  \SetKwInOut{Output}{Output}
  \Input{$n_{\mbox{\scriptsize row}} \times n_{\mbox{\scriptsize col}}$ cores in rectangle with local partial-sum PS$(i, j)$.}
  \Output{Network trace $\mathbf{N}$}
  $\mathbf{N} \leftarrow \emptyset$\;
  $\mbox{fold} = \lceil\log_2^{n_{\mbox{\scriptsize row}}}\rceil$\;
  \For{($f\leftarrow 1; f < 2^{\mbox{\normalfont \scriptsize fold}}; f=f*2)$}
  {
    %\tcc{Ops in each L execute in parallel.}
  	$\mathbf{L}\leftarrow \emptyset$\;
    \For{($i=f; i<n_{\mbox{\normalfont\scriptsize row}}; i=i+2*\mbox{\normalfont fold} $)}{
    	\For{$j=0, \ldots, n_{\mbox{\scriptsize \normalfont col}} $}{
            	$\mathbf{L}$.add(``Send PS$(i, j)$ FROM $(i, j)$ TO $(i-\mbox{fold}, j)$'')
        }
    }
    $\mathbf{N}$.add($\mathbf{L}$)\;
    $\mathbf{L}\leftarrow \emptyset$\;
    \For{($i=f; i<n_{\mbox{\normalfont\scriptsize row}}; i=i+2*\mbox{\normalfont fold} $)}{
    	\For{$j=0, \ldots, n_{\mbox{\scriptsize \normalfont col}} $}{
            	$\mathbf{L}$.add(``Add PS$(i, j)$ TO PS$(i-\mbox{fold}, j)$'')
        }
    }
    $\mathbf{N}$.add($\mathbf{L}$).
  }
  
  \Return $\mathbf{N}$\;
\end{algorithm}


2. {\em Mapping convolution layers}:
For a convolution layer with input size $h\times w \times c_{\mbox{\scriptsize in}}$ and kernel size $k\times k \times c_{\mbox{\scriptsize in}}\times c_{\mbox{\scriptsize out}}$, we need $n_h \cdot n_w$ cores to cover the spatial dimension $h\times w$ where $n_h = \lceil h/(\sqrt{N_{\mbox{\scriptsize in}}}-2(k-1))\rceil$ and $n_w = \lceil w/(\sqrt{N_{\mbox{\scriptsize in}}}-2(k-1))\rceil$. So, to cover all input and output channels, a total of $c_{\mbox{\scriptsize in}}\cdot c_{\mbox{\scriptsize out}}\cdot n_h \cdot n_w$ cores is needed. The weights are mapped so that each neuron performs the convolution in one channel as its partial sum.

To produce the convolution sum, along each channel, the neighbouring cores first exchange their partial-sums to produce the convolution of the boundary pixels. Then, among the channels, the partial sums are accumulated to complete the convolution.
\begin{comment}
\begin{figure}[ht]
\includegraphics[width=\linewidth]{Figures/cnn_noc.pdf}
\caption{Partial-sum NoC for Convolution.}
\label{fig:cnn_noc}
\end{figure}
\end{comment}
As a convolution layer scans through the input image, there will be overlap at the boundary of each core.
%For instance, computing the output in the corner shown as red box requires input from all four cores. These overlapped data has to be duplicated and supplied to each of the four in a conventional mapping.

As an example, to map a $3\times 3$ kernel over an MNIST image to cores of $256$ synapses and $256$ neurons (Figure~\ref{fig:conv_map}), we split the $28\times28$ input into four $14\times 14$ rectangles and allocate each quadrant to a core, as shown in (a). Computing the output in the overlapping corners of each core, highlighted in a red box, requires input from all four cores. These overlapped data has to be duplicated and supplied to each of the four. In this example,
each core produces $12\times 12$ complete weighted sums (green areas), slices of $2\times 12$ partial sums at each of the four boundaries and $2\times 2$ partial sums at each of the four corners. At the boundary of core (0,0) and (0,1), sending (0,1)'s outer partial sum~(A) to (0,0) and adding to its inner partial sum~(B) will produce the complete sum with size $1\times 12$. At the corner, sending the partial sums~(C, D, E) to (0,0) and adding to F will produce the complete sum of size $1\times 1$. The operations are symmetric among the neighboring cores. As a result, each core produces $14\times 14$ outputs. 

The partial sums in Figure~\ref{fig:conv_map} (A-F) are routed by the partial sum NoCs, where the data to be accumulated must be produced by the neurons in the same channel, e.g. areas (C-F) must be produced by neuron \#1 of all four cores. Consider F' area in core (1,1). Since area D has occupied neuron \#1, F' has to be allocated to a different neuron from F. This requirement applies to all partial sum areas and results in an inter-changing pattern of neuron allocation among neighboring cores.
\begin{figure}[t]
\includegraphics[width=0.65\linewidth]{Figures/cnn_map.pdf}
\caption{Mapping of a convolution layer, (a) viewed in 2D data and (b) mapped onto 4 Shenjing cores.}
\label{fig:conv_map}

\end{figure}

3. {\em Mapping ResNet shortcuts}: Converting ResNet to its spiking version was proposed in~\cite{Hu_spike_resnet} where a layer's output skips its following residual block and directly adds to the block's output as a shortcut. In SNN, the shortcut needs to be normalized so we add a  normalization layer in Shenjing with weights set to a diagonal matrix $\text{diag} (\lambda)$. The partial sum after normalization is then sent to the corresponding cores of the residual block through PS NoCs for addition. Shenjing's PS and spike NoCs naturally support ResNet-style shortcuts between non-adjacent cores, through intermediate routers. 

\noindent{\bf Logical spike NoC mapping.}
In general, the mapping of spike NoCs among layers is straightforward because the output size of cores naturally fit the input size. So, we usually just give a core-to-core mapping. However, when the output size of each core in a layer is small enough, multiple cores' output can be directed to one core in the subsequent layer. For this purpose, we map the output of multiple cores to different non-overlapping neurons so they can be sent to the same core.
\begin{comment}
Here we explain the mapping of spikes from the pooling layer to the convolution layer as an example. As the pooling layer reduces the spatial dimension of input data by kernel size and stride, it also reduces the number of cores required for the subsequent convolution layer.


Suppose we direct the $14\times 14$ output of each core in Figure~\ref{fig:conv_map}(b) to four pooling cores with kernel and stride $2\times 2$, each core will then produce $7\times 7$ pooling outputs. Output of all the four cores will be routed to the input of one core in the following convolution layer. Therefore, they need to be allocated to different and non-overlapping neurons. 
\end{comment}

\begin{comment}
\begin{figure}[tbh]
\includegraphics[width=0.9\linewidth]{Figures/floorplan2.png}
\caption{Floorplan and area breakdown of a single Shenjing tile.}
* The 128-neuron clusters corresponding to each SRAM bank are combined vertically to form 256 neurons finally
\label{fig:floorplan}
\end{figure}
\subsection{Physical mapping: Core allocation and control signal generation }
\end{comment}

%{\color{blue}
%The authors claim that the primary focus of their work is reducing on-chip movement of data. Are there factors other than neuron core size which affect movement of data on the chip? E.g. Relative placement of layers on to cores during the mapping phase.
%}

\noindent{\bf Physical Mapping.}
For every layer, the logical cores are then mapped to the Shenjing architecture. We implemented a greedy algorithm to allocate adjacent layers next to each other, while attempting to minimize the number of chips (of 784 cores each) used and the cost of data movement. In particular, for each layer, we first search for a rectangular space that can accommodate this layer among existing chips.
If that is not available, we then add Shenjing chips to house this layer.
For the physical routing of the logical NoC schedule, we use simple deterministic XY routing. For flow control, a packet (spike or PS) is scheduled to wait if the output port/link is occupied, as there are no buffer queues. After physical mapping, a cycle-by-cycle compiled schedule of atomic operations onto binary signals that control Shenjing's hardware components (see Table~\ref{table:op2sig}) is generated.    %{\bf Peh: Do you ever have multi-hop routing? If so, do you assume a fixed X then Y? What if the entire multihop is not fully available? You block at the source router?}



\begin{table}[t]
\centering
\footnotesize
\vspace{-1em}
\begin{tabular}{|l|l|}
\hline
\multirow{2}{*}{\textbf{Partial Sum Router}} & \textbf{type{[}2{]}}  \textbf{sum\_buf}   \textbf{add\_en} \\            
& \textbf{consec\_add}  \textbf{bypass}        \textbf{in\_sel{[}2{]}}  \textbf{out\_sel{[}3{]}} \\ \hline
{\tt SUM \$SRC, \$CONSEC}&            {\tt 00}                      {\tt 0}                   {\tt 1}                            {\tt \$CONSEC}              {\tt 0}                      {\tt \$SRC}                     {\tt 000}                        \\ \hline
{\tt SEND \$SRC, \$DST}            & {\tt 00}                      {\tt \$SRC}               {\tt 0}                            {\tt 0}                     {\tt 0}                      {\tt 00}                         {\tt \$DST}                      \\ \hline
{\tt BYPASS \$SRC, \$DST}          & {\tt 00}                      {\tt 0}                   {\tt 0}                            {\tt 0}                     {\tt 1}                      {\tt \$SRC}                      {\tt \$DST}                      \\ \hline\hline
\multirow{2}{*}{\textbf{Spike Router}}       & \textbf{type{[}2{]}}  \textbf{spike\_en}  \textbf{sum\_or\_local}     \\ 
& \textbf{inject\_en}   \textbf{bypass}        \textbf{in\_sel{[}2{]}}  \textbf{out\_sel{[}2{]}} \\ \hline
{\tt SPIKE \$SUM\_OR\_LOCAL}                & {\tt 01}                      {\tt 1}                   {\tt \$SUM\_OR\_LOCAL}                        {\tt 0}                     {\tt 0}                      {\tt 00}                         {\tt 00}                         \\ \hline
{\tt SEND \$DST}                 & {\tt 01}                      {\tt 0}                   {\tt 0}                            {\tt 1}                     {\tt 0}                      {\tt 00}                         {\tt \$DST}                      \\ \hline
{\tt BYPASS \$SRC, \$DST}          & {\tt 01}                      {\tt 0}                   {\tt 0}                            {\tt 0}                     {\tt 1}                      {\tt \$SRC}                      {\tt \$DST}                      \\ \hline\hline
\multirow{2}{*}{\textbf{Neuron Core}}             & \textbf{type{[}2{]}}  \textbf{r\_weight}  \textbf{w\_weight{[}4{]}}    \\   
& \textbf{acc{[}4{]}}      \textbf{pad{[}5{]}}                          \\ \hline
{\tt LD\_WT}                       & {\tt 10}                      {\tt 0}                   {\tt 1111}                                         {\tt 0000}                {\tt 00000}             \\ \hline
{\tt ACC}                         & {\tt 10}      {\tt 1}                                 {\tt 0000}                                        {\tt 1111}            {\tt 00000}                     \\ \hline
\end{tabular}


\caption{Mapping of atomic operation to hardware control signals. \newline
{\normalfont There are three types of atomic operations for partial sum router, spike router and neuron core, defined by the first 2 bits. {\tt \$SRC} and {\tt \$DST} are one of {\tt N}(orth), {\tt S}(outh), {\tt E}(ast), or {\tt W}(est). {\tt \$CONSEC} controls the multiplexor in Figure~\ref{fig:core_ps_spike}~(b) that feeds either the local PS value (0) or the previous sum (1) as the first operand into the adder.}}
\label{table:op2sig}
\end{table}



==> Arxiv-Shenjing with app/related-works.tex <==
%{\color{blue}
%How does this mapping of SNN compare with other mapping technique introduced in [R1].
%
%For ANN, there are many optimization techniques such as pruning, compression, and quantization, etc. Are these compatible or can be implemented equivalently in the proposed SNN architecture? Also, some quantitative comparison between the proposed SNN with other ANNs that are equipped the above optimization techniques would be very helpful.
%}

% Update Table 7 for rebuttal
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[tb]
\footnotesize
\vspace{-1em}

\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
 Architecture                        & Tech            & Accu. & FPS                   & Voltage     &Power& uJ/\\

& (nm)&   & & &(mW) &Frame\\ \hline

 SNNwt~\cite{du2015neuromorphic}                       & 65                  & 91.82\%  & N.A.                    & 1.2V        &N.A.& 214.7                                                                   \\ \cline{1-7} 
 

    SpiNNaker                       & 130                  & 95.01\%  & 77                    & 1.8V/        &300& 3896     \\ 
    ~\cite{spinnaker}& &   & &1.2V & & \\ 
\cline{1-7} 

 Tianji~\cite{ji2018bridge}                       
  & 120                 & 96.59\%  & N.A.                    & 1.2V        &120*& N.A.                                                          \\ \cline{1-7} 

 TrueNorth   & \multirow{2}{*}{28} & 92.70\%  & \multirow{2}{*}{1000} & \multirow{2}{*}{0.775V}      & 0.268 &0.268                                                                 \\ \cline{3-3} \cline{6-7} 
 ~\cite{esser2015backpropagation} &                       & 99.42\%  &           &                     & 108 &108                                                                   \\ \cline{1-7} 
 {\it This work }                      & {\it 28}                  & {\it 96.11\%}  & {\it 40}                    & {\it 1.05V/} & {\it 1.26} & {\it 38}                                                                    \\ 
     & &   & & {\it 0.85V} & & \\ 
\hline
\end{tabular}
* is only dynamic power.
\caption{Comparison with existing SNN architectures for MNIST MLP}
\label{table:hardware-comparison}
\end{table}

The field is huge so we can only focus on SNN accelerators and NoCs in neural network chips here.

\noindent
{\bf SNN Hardware.} 
Apples-to-apples comparison with prior SNN architectures is difficult especially when we do not have access to others' models and implementations.
%input model differs in dataset, network structure, pre-trained accuracy, frames-per-second; while hardware differs in technology node, frequency, circuits. 
Table~\ref{table:hardware-comparison} is our best-effort comparison with existing SNN architectures for MNIST benchmark. 
The spatially expanded SNNwt~\cite{du2015neuromorphic} is an application specific architecture where input size of neurons are precisely 784, hence avoiding the partial-sum issue, but it will not scale. SpiNNaker~\cite{spinnaker} uses 20 ARM cores to implement neurons and facilitates communication with two specialized NoCs. One NoC handles inter-chip communication in a 2D triangular toroidal mesh and the other handles communication between cores and peripherals.
Loihi~\cite{loihi}, like SpiNNaker, uses conventional CPUs and hence incurs high power. 
%However, none of them explicitly resolve the partial-sum issue.
%For other benchmarks like Cifar-10, there are too many differences in the network models that the comparison may not be meaningful. 

IBM's TrueNorth fabricated 4096 cores connected by a mesh NoC~\cite{truenorth}. Due to the rigid 256$\times$256 input/output constraints of each core, migrating any neural net to TrueNorth requires much restructuring and retraining of the model, often ending up using more resources. In fact, TrueNorth has its own programming paradigm and simulator~\cite{amir2013cognitive} that users have to program, train and optimize for. Energy is highly correlated with accuracy in TrueNorth: its power increases by 402$\times$ when the MNIST accuracy is boosted from 92.7\% to 99.42\% (from Figure 3C of~\cite{esser2015backpropagation}) because a different model had to be used. Shenjing achieves an accuracy of 96.11\% when running MNIST, with energy that is an order of magnitude lower than SNNwt~\cite{du2015neuromorphic}, comparable to TrueNorth. %{\bf WB: no power number reported in [10] and no fps so we can't calculate it from energy}
%{\bf Peh: [10] has no power number in table?}
For CIFAR-10, with significant manual tuning, TrueNorth produces 83.41\% accuracy with 4042 cores at 204.4 mW~\cite{Esser11441}. In comparison, we simply automatically map an existing neural net using 2977 cores and achieved a 75.9\% accuracy close to that of the original ANN version. Shenjing consumes a higher 664.20 mW, a large portion of that (47\%) is consumed by the SRAMs. 
Implementation wise, TrueNorth adopts custom SRAMs and circuit layouts at lower voltage and mixed asynchronous-synchronous circuits, while Shenjing uses the foundry's memory-compiled higher-VDD SRAMs and fully synthesized clocked circuits.
%leading to 128 13-bit adders synthesized for each sub core, and (128*4+256=768) adders in each neuron core. This results in our neuron core (SRAM+accumulators) taking up 97.6\% of Shenjing's total power in the MNIST MLP application. 
%Custom designed SRAMs with in-memory compute such as~\cite{VermaJSSC2017} will substantially reduce Shenjing's power, and is orthogonal.

Ji et. al.~\cite{ji2018bridge} proposed a software mapping tool that takes ANN/SNN models and automatically transforms and maps them onto hardware accelerators taking into account hardware constraints. They demonstrated mapping of ANNs onto the Tianji SNN accelerator~\cite{shi2015development}, enabling transfer learning of trained ANN models. However, without partial sum support in the NoCs, they have to transform the neural nets substantially for good accuracy. Shenjing's NoCs enable the hardware to realize same accuracy as the original abstract SNN model, simplifying mapping. The recent Tianjic chip~\cite{pei2019towards}, which we believe is the further development of~\cite{shi2015development}, configures cores into ANN, SNN or hybrid mode. It handles sums across cores by configuring some cores into hybrid mode and adding an extra ANN layer for accumulation. Compared to Shenjing's PS NoCs, this approach lowers core utilization for computing and requires restructuring of SNN models. The 156-core Tianjic chip consumes 0.95W.
%operates asynchronously, like TrueNorth~\cite{Merolla2014TrueNorth}, where each core has a single neuron to mimic multiple neurons in time division multiplexing fashion. 

%Other notable SNN hardware includes %SpiNNaker~\cite{spinnaker} and Intel's Loihi~\cite{loihi} which use conventional CPUs and hence incur high power, and custom accelerators INXS~\cite{inxs} and Neurogrid~\cite{benjamin2014neurogrid}.
%, and Tianji~\cite{shi2015development}. 

% and consumed 65mW for a typical recurrent neural network

\noindent
%{\bf ANN Hardware.} There are many custom hardware chips for ANNs. Eyeriss~\cite{Chen2016} is one of the first ANN accelerator. It achieves a high energy efficiency of 236mW for VGG-16 if a low throughput of 0.7~FPS is acceptable. A power of 320mW and 596mW was achieved for ShiDianNao~\cite{du2015shidiannao}, respectively. {\bf Peh: Why 2 numbers? Any MNIST numbers so we can compare?}
%A 64 core EIE~\cite{han2016eie} designed for ``deep compression'' networks consumes 590mW.

\noindent
{\bf Related NoCs.} Prior NoCs in SNNs for delivering spikes are routed dynamically. Hence, spike trains may not be delivered in global order to all neuron cores, causing errors in spiking. Prior works tackle this with a fixed-latency interconnect~\cite{embracepc2013} or by a hardware ordering mechanism within the NoC~\cite{oridac2017}. 
Shenjing's spike NoC is software-scheduled, and the scheduling algorithm ensures ordering of the spikes so the routers do not need to handle ordering.
Computation in NoCs has been proposed in~\cite{kwon2018maeri}, configuring adder switches at run-time to support arbitrary sizes for DNN partition and mapping whilst our adders in partial sum NoCs are fixed. %The former is more complicated in terms of configuration and control than ours. ~\cite{he2018asynchronous} implements a Booth multiplier into an asynchronous mesh routing network so as to share the computing capability. ~\cite{yang2018optimal} integrates STT-RAM and SRAM buffers in routers for simple logic operations to reduce the computation overhead on processors.




==> Arxiv-Shenjing with app/results-arch.tex <==


%This section explores the architectural design space of Shenjing and the implementation tradeoffs based upon synthesized timing, power and area numbers. 
We implemented our design in system Verilog and synthesized it into gate-level netlist on a 28nm process. We focus on MNIST in this section due to RTL simulation tractability; Larger network results are shown in the next section.
%of a full RTL implementation of Shenjing. We implemented our design in system Verilog HDL and verify its functionality using Synopsys VCS tool. We run synthesis with Design Compiler to synthesize RTL into gate-level netlists in a commercial 28nm CMOS process.
%Throughout this section, for RTL simulation tractability, we focus on the small MNIST MLP SNN example of Figure~\ref{fig:neuron_core_abstract}(b). Simulation results of larger networks are presented in the next Section 6.

\noindent{\bf Area.} Each tile (neuron core + NoC routers) in Shenjing is synthesized at supply voltages of 0.85V for logic gates and 1.05V for SRAMs, respectively, into 0.262 million logic gates with a total cell area of 0.49 mm\textsuperscript{2}. 
%Each square tile thus has a dimension of 0.7mm by 0.7mm. 
We assume a maximum die size of 20mm by 20mm, so 784 Shenjing tiles can be fit onto a chip in a 28-by-28 grid.  
%Figure~\ref{fig:floorplan} illustrates the floorplan and area breakdown of the tile. 
Our routers take up a sizable portion of tile area (39\%), comparable to the SRAMs (44\%) as they perform computations of sum and spikes as well.

\begin{figure}[tb]
\includegraphics[width=0.8\linewidth]{Figures/fps_freq_pwr.pdf}
\vspace{-0.5cm}
\caption{Tradeoff of Shenjing's overall throughput with clock frequency and power of a single tile (neuron core + NoC routers)}
\label{fig:fps_freq_pwr}
\end{figure}

\noindent{\bf Interactions of neural net throughput with circuit timing and power.} The critical path begins from the accumulative registers in the neuron circuit and ends at the pooling registers located in the IF/Spiking logic. %(Figure~\ref{fig:core_ps_spike}~(c)) with a delay of 4.11 ns. Hence, 
The maximum achievable frequency of Shenjing is 243MHz. 
%As the SRAM in each subcore takes multiple cycles to complete a read, there is a 144-stage (128-stage for memory read and 16-stage for accumulation, addition and spiking) pipeline for the computation of the first fully connected layer FC1 and its output propagating before the neuron core can accept a new set of inputs. 
Our work is targeted to process the FC and convolutional layers at a minimum throughput of 30 frames/sec (fps) which suffices for typical video applications deploying CNNs. 
%Hence for MLP and CNN datasets, the pipeline latency and the throughput determine frequency as $F_{\mbox{\scriptsize req}} = \mbox{fps} \times (\mbox{ts} + \mbox{nl}) \times \mbox{pc}$
%where \textit{ts} is time steps of an input spike train, \textit{nl} is the number of layers to be executed after this layer, \textit{pc} is the number of pipeline cycles. For the MLP walkthrough example, a frequency of 120~kHz works given \textit{ts}, \textit{nl} and \textit{pc} are 20, 1 and 144, respectively. However, for the CNN and CIFAR-10 networks, the frequency has to be increased significantly as more cycles (\textit{pc}) are required in the convolutional layer to handle the substantial spike bandwidth required. 
Complexity of the SNN model impacts the chip frequency needed to achieve this. Figure~\ref{fig:fps_freq_pwr} shows the tradeoff of throughput with frequency and power of a tile. 
%We choose various mainstream video frame rates such as 24fps, 30fps, 35fps, 40fps and 60fps for comparison. 
As throughput is increased from the 24 to 60fps, the required operating frequency ($F_{req}$) increases from 73kHz to 181kHz. Power  dissipation scales linearly with $F_{req}$, increasing $2.48 \times$ from 139$\mu$W to 235$\mu$W.
Here we chose a target video throughput of 40fps for MNIST MLP for a balance of power and performance. 

\begin{comment}
\begin{figure}[ht]
\includegraphics[width=\linewidth]{Figures/core_vs_links.pdf}
\caption{Number of NoC links and corresponding NoC power with increasing neuron core size.} 
\label{fig:core_vs_link}
\end{figure}
\end{comment}

%{\bf Architectural exploration of core and subcore size.} We explore the design space of Shenjing's core microarchitecture in terms of performance, throughput and power in order to pin down appropriate NoC and neuron core parameters. In Shenjing, a core size of $m \times n$ is defined by the number of spike inputs (\textit{m}) it can take and the number of neurons (\textit{n}) it accommodates. At one extreme, a single neuron can constitute a neuron core, so all accumulation occurs in the huge network, outside the core. On the other end of the spectrum, the entire Shenjing can consist of a single core, so all accumulation is performed in-memory. By exploring neuron core size from 512 down to 1, the NoC overhead grows drastically. Specifically, in our MNIST example, with single-neuron cores, the output spikes from FC1 layer cores to FC2 cores will cross 512 router hops instead of the original 2 hops with 256-neuron cores. % {\bf Wang Bo: Instead of power per NoC link, which correlates with number of NoC links, do we want the energy of a per-neuron add which consists of in-memory adds + in-network adds instead? I thinks the active energy is the same as when neuron core size shrinks the accumulator/add bitwidth shrinks too.} 
%Figure~\ref{fig:core_vs_link} measures this overhead in terms of NoC links and corresponding NoC power for the MLP example. By scaling up the dimension from $1 \times 1$ to $512 \times 512$, NoC link power reduces by $784641 \times$. 


%\begin{figure}[tbh]
%\begin{minipage}{0.7\linewidth}
%\includegraphics[width=\linewidth]{Figures/core_util_size.pdf}
%\end{minipage}
%\begin{minipage}{0.28\linewidth}
%\includegraphics[width=\linewidth]{Figures/core_util.pdf}
%{\tiny An $N\times N$ kernel mapped as a blue rectangle along SRAM column.}
%\end{minipage}
%\caption{Core utilization of different neuron core sizes with respect to CNN kernel size\vspace{-10pt}}
%\label{fig:core_vs_utilization}
%\end{figure}

%However, the number of neurons per core is capped by SRAM utilization. Firstly a squarish dimension is preferred in our work to ease mapping as the input and the output counts of FC layers are usually similar in the models. Secondly, when $k \times k$ window in a CNN kernel is mapped to a neuron as Figure~\ref{fig:core_vs_utilization}, the corresponding weights are all stored along a SRAM column where $k \times k \div column\_length$ of SRAM cells are in use. 
%Therefore, if the size expands from $256 \times 256$ continuously, SRAM utilization diminishes as most kernel windows in our models do not exceed $5 \times 5$. Figure~\ref{fig:core_vs_utilization}
% shows $256 \times 256$ is a moderate dimension when trading off network complexity and SRAM utilization, which is our choice of neuron core size.
 

 
%\begin{table}[bh]
%\centering
%\small
%\caption{Impact of subcore dimension.}
%\label{table:subcore}
%\begin{tabular}{|c|S[table-format=3.0]|S[table-format=3.0]|S[table-format=6.0]|} 
%\hline
%{\bf Subcore} & \multicolumn{1}{c|}{\bf Pipeline} & \multicolumn{1}{c|}{\bf Freq at} & \multicolumn{1}{c|}{\bf Extra area}\\
%{\bf size} & \multicolumn{1}{c|}{\bf stage} & \multicolumn{1}{c|}{\bf 40 fps (kHz)} & \multicolumn{1}{c|}{($\mu \mbox{m}^2$)} \\ \hline
%$32\times 32$                                                 & 32                                                        & 40                                                            & 153600                                                       \\ 
%\hline
%$64\times 64$                                                 & 64                                                        & 67                                                            & 76800                                                        \\ 
%\hline
%$128\times 128$                                               & 128                                                       & 120                                                           & 38400                                                        \\ 
%\hline
%$256\times 256$                                               & 256                                                       & 228                                                           & 0                                                            \\
%\hline
%\end{tabular}
%\vspace{-0.1cm}
%\end{table}

%In addition, we also chose the subcore size carefully to further improve area-performance. As Table~\ref{table:subcore} shows, a $256 \times 256$ core can be decomposed into 4 $128 \times 128$ or 16 $64 \times 64$ or 64 $32 \times 32$ subcores. Each division halves the number of pipeline stages as more subcores can run in parallel, thus reducing the required $F_{req}$ for a fixed \textit{fps}. We picked 4 subcores to balance timing and area overhead.  

 






 


\begin{table}[bt]
\footnotesize
\vspace{-1em}

\begin{tabular}{|l|l|S[table-format=1.4]|S[table-format=3.2]|}
\hline
\multicolumn{1}{|c|}{\textbf{Block}}                                                                         & \multicolumn{1}{c|}{\textbf{Atomic Op}} & \textbf{\begin{tabular}[c]{@{}c@{}}Active power\\ @120~kHz \\ (mW)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Active energy\\ per neuron\\ (pJ)\end{tabular}} \\ \hline
\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Partial sum\\ router\end{tabular}}} & SUM             & 0.0383                                                                          & 1.25                                                                               \\ \cline{2-4} 
                                                                                       & SEND            & 0.0443                                                                          & 1.44                                                                               \\ \cline{2-4} 
                                                                                       & BYPASS          & 0.0455                                                                          & 1.48                                                                               \\ \hline
\multirow{3}{*}{\textbf{Spike router}}                                                 & SPIKE           & 0.0689                                                                          & 2.24                                                                               \\ \cline{2-4} 
                                                                                       & SEND            & 0.0721                                                                          & 2.35                                                                               \\ \cline{2-4} 
                                                                                       & BYPASS          & 0.0381                                                                          & 1.24                                                                               \\ \hline
 \textbf{Neuron core$^1$}                                                                                         & ACC$^2$             & 0.0412                                                                          & 171.67                                                                             \\ \hline
\textbf{Initialization}                                                       & LD\_WT$^2$          & 0.0568                                                                          & 236.67                                                                             \\ \hline
\end{tabular}
\caption{Synthesized active power and energy of atomic operations}

$^1$ SRAM power was obtained at 1.05V while the other logic operates at 0.85V due to the limitations of the SRAM libraries we have access to.\\
$^2$ Active energy of LD\_WT (loading of weights) which occurs only once during initialization, and ACC (accumulation across a subcore) is higher as these operations take 131 cycles while the others take a cycle.
\label{table:energy}
\end{table}


\noindent{\bf Power.} We performed cycle accurate power analysis using Prime Time PX for MNIST MLP running on 10-core Shenjing and the overall power reported by the tool was 1.26mW. %{\bf Sleep mode and clock gating techniques are applied to optimize the leakage power.}
%Unless we want to discuss breakdown of leakage and dynamic: while the dynamic power was 0.23mW. %SRAM consumed 45.8\% of the total power, and 51.5\% of leakage power. Neurons including accumulators accounted for 7\% total power, while the partial sum and spike routers dissipated 36\% and 9.4\% of total power, respectively. {\bf Peh: Table 5 and this accompanying text is confusing: SRAM is labeled as within the Neuron core, which takes up bulk of power, but yet here it says Neurons take up 7\% power. Indicate what's considered Neurons -- ACC? SRAM -- LD\_W? I'm adding some explan ation of our high LD and ACC power in Discussion.}

Table~\ref{table:energy} lists each atomic operation's energy by PrimeTime with the switching activity of MNIST MLP (6.25\%), calculated using average number of spiking axons per core in each time step. %Peh: no longer 50% switching
%Table~\ref{table:energy} shows the estimated total power of 1.52mW (dynamic power 0.375mW, leakage 0.115mW), which is just 4.8\% off the circuit-level power estimate with PrimeTime.
%while leakage power is 0.115mW for the tile. 
These RTL power estimates are fed into our system-level functional simulations for power estimation of larger networks.


==> Arxiv-Shenjing with app/results-system.tex <==

We developed a cycle-level functional simulator for simulating large scale neural network benchmarks that are beyond the ability of detailed RTL simulation. It is aimed to be cycle-by-cycle equivalent to RTL simulation in (1)~running input atomic operations as defined in Table~\ref{table:op2sig}, (2)~producing and routing data in neuron cores and NoCs, and (3)~providing execution statistics for deriving architectural power estimates.

\begin{table}[ht]
\centering
\footnotesize
\vspace{-1em}

\begin{tabular}{|c|c|c|c|}
\hline
{(a) MNIST}
& {(b) MNIST} 
&{(c) CIFAR-10}
&{(d) CIFAR-10}\\
{MLP}
& {CNN} 
&{CNN}
&{ResNet} \\ \hline

\hspace{-0.6em}\begin{tabular}[c]{@{}l@{}}Input(28, 28, 1)\\ FC1(784, 512)\\ FC2(512, 10)\end{tabular} \hspace{-0.8em}
&\hspace{-0.6em}\begin{tabular}[c]{@{}l@{}}Input(28, 28, 1)\\ Conv1(3,3,1,16)\\ Pool1(2,2)\\ Conv2(3,3,16,32)\\ Pool2(2,2)\\ FC1(1568, 128)\\ FC2(128, 10)\end{tabular} \hspace{-0.8em}
&\hspace{-0.6em}\begin{tabular}[c]{@{}l@{}}Input(24, 24, 3)\\ Conv1(5,5,1,16)\\ Pool1(2,2)\\ Conv2(5,5,16,32)\\ Pool2(2,2)\\ Conv3(3,3,32,64)\\ Pool3(2,2)\\ FC1 (576, 256)\\ FC2(256, 128)\\ FC3(128, 10)\end{tabular} \hspace{-0.8em}
& \hspace{-0.6em}\begin{tabular}[c]{@{}l@{}}Input(24, 24, 3)\\ Conv1(5,5,1,16)\\ Pool1(2,2)\\ $	\overline{\mbox{Res/Conv1(5,5,16,32)}}$\\Res/Conv2(5,5,32,32)\\ \underline{Res/Conv3(5,5,32,32)}\\ Pool2(2,2)\\ Conv3(3,3,32,64)\\ Pool3(2,2)\\ FC1(576, 256)\\ FC2(256, 128)\\ FC3(128, 10)\end{tabular} \hspace{-0.8em}

\\ \hline
\end{tabular}
\caption{Summary of Applications.}
\label{table:applications}
\end{table}


With these requirements, we implemented the Shenjing components in Java. %The neuron core is implemented in abstract because it always operates as a whole. 
The partial-sum and spike NoCs of the functional simulator are essentially the corresponding RTL modules with all the details of registers, wirings, crossbars etc. rewritten in Java.
We verified this functional simulator against our RTL simulator, automatically checking the state of each component cycle by cycle given the same input instructions and data.  We have also verified our power estimation against the RTL simulation using the MNIST-MLP benchmark.

%\noindent {\bf Benchmark power-performance.}
We simulate Shenjing with MNIST and CIFAR-10 datasets on 4 neural network structures, covering the most common neural network layers including convolution, average pooling, fully connected and residual block. %The results are shown in Table~\ref{table:benchmark}. 
%{\color{blue}
%The overall power consumed by different neural networks mapped on Shenjing seems to consist of neuron core power only (as shown in Table 6). Taking the inter-core communication power into consideration would give a more accurate picture of its efficiency and scalability aspects.
%}



%As explained in Section~\ref{sec:need-PS-Noc}, the loss of accuracy is from ANN-to-SNN conversion, and there is no further loss when implementing the SNN model on Shenjing. 
%The total power and power per core reported includes the cost of inter-chip communication. %Peh: This should already be mentioned in Section 2.  For MNIST MLP, we implement the network on a TrueNorth like architecture without partial sum NoCs~\cite{lee2019system}, and the accuracy drops to 93.61\%. It also requires five more cores for merging spikes from multiple cores.


%{\color{blue}
%could the authors provide a baseline experiment to show how much accuracy is potentially lost without the adder tree in the NOCs.
%If the technology node used is the same, how would Shenjing compare to TrueNorth given the same network (or as similar as possible) is mapped on both?
%}



\begin{table}[tb]
\centering
\footnotesize
\vspace{-1em}
\begin{tabular}{|c|c|c|c|c|}
\hline
         & MNIST  & MNIST  & CIFAR-10 & CIFAR-10 \\ 
         & MLP    & CNN    & CNN     & ResNet  \\ \hline
ANN Accu. & 0.9967 & 0.9913 & 0.7992  & 0.7825  \\ \hline
Abstract SNN Accu.  & 0.9611 & 0.9715 & 0.7590  & 0.7250 \\ \hline
Shenjing Accu. & 0.9611 & 0.9715 & 0.7590  & 0.7250  \\ \hline
\#Cores  & 10    & 705    & 2977    & 5863  \\ 
  &      &     & (4 chips)    & (8 chips)  \\ \hline
Timestep (T)      & 20     & 20    & 80      & 80      \\ \hline

Frames per sec      & 40     & 30    & 30      & 30      \\ \hline

Frequency& 120~kHz & 207~kHz     & 1.25~MHz    & 2.83~MHz    \\ \hline
Power (mW)& 1.35     & 87.54   & 456.71    & 887.81   \\ \hline
Power/Core (mW)& 0.135     & 0.124   & 0.153    & 0.151   \\ \hline
mJ/frame& 0.038   & 2.92      & 15.22    & 29.59  \\ \hline
Mapping time(ms)& 660   & 2142      & 4384    & 12022  \\ \hline 
\end{tabular} 
*Timestep is the length of spike train for each image.
\caption{Overall Performance.}
\label{table:benchmark}
\end{table}

\noindent
%{\bf Peh: Need to explain SNN's downside here of accuracy loss, then defend with numbers in Table VI extended to a huge network}
{\bf Accuracy.} 
Table~\ref{table:benchmark} reports the accuracy of the original ANN model, the converted abstract SNN model, and the SNN model when implemented on Shenjing. 
SNN's use of binary instead of full precision floating point data brings about a loss in accuracy. This is the main disadvantage of SNNs. However, for most applications, the amount of accuracy loss is usually acceptable. In fact, there is substantial research on reducing the resource requirements of ANNs at the cost of accuracy loss.

MNIST: We built both a fully connected as well as a CNN network for MNIST as shown in Table~\ref{table:applications}(a-b). 
As MNIST is a relatively simple dataset, both networks achieved high accuracy when trained as ANN. The converted SNN suffers just 3\% loss in accuracy before mapping to hardware, with no additional loss after mapping onto Shenjing. 
%{\bf Peh: cite why this is comparable :P}

CIFAR-10 CNN:
CIFAR-10 is a dataset of 60,000 $32\times32$ color images in 10 classes, 6000 each. The image size was first reduced to $24\times 24$ by center cropping. We built a conventional CNN and a residual CNN for it following the methods described in~\cite{Cao2015} as shown in Table~\ref{table:applications}(c). The resultant SNN achieved an accuracy of 75.90\%, while the ANN accuracy was 79.92\%.
%In~\cite{Cao2015}, the converted accuracy was claimed to be 77.43\%. The loss of accuracy comes mainly from the low precision of our choice of 5-bit weights. When we increase the precision of the weights to 9 bits, accuracy improved significantly to 79.20\%, only 0.72\% less than the ANN. 
%We will discuss the trade-off of accuracy versus area and power in Section~\ref{sec:discuss-precision}.
%Peh: I think this will be discussed in Section 5 through RTL as well?


CIFAR-10 ResNet: Residual network (ResNet)~\cite{he2016deep} is designed to solve the degradation problem in training very deep CNNs. In this benchmark, we demonstrate that Shenjing supports ResNet using a small scale network as in Table~\ref{table:applications}(d).
To the best of our knowledge, this is the first demonstration of a SNN hardware that can be configured automatically to run residual networks, thanks to Shenjing's NoCs.

\noindent
{\bf Mapping time.} Our toolchain automatically mapped all the above ANNs onto Shenjing. %Mapping is done offline and the time is shown in Table~\ref{table:benchmark}. 
The mapping for the largest network took 12 seconds on an Intel Core i7-8550U CPU.

\noindent
{\bf Power.}
Table~\ref{table:benchmark} shows our architectural power estimates. %Moved to RTL section
%Table~\ref{table:energy} lists each atomic operation's energy as obtained through RTL simulation assuming the switching activity of MNIST MLP (6.25\%), calculated using the average number of spiking axons per core in each time step of the MNIST benchmark. %Peh: no longer 50% switching
%Table~\ref{table:energy} shows the estimated total power of 1.52mW (dynamic power 0.375mW, leakage 0.115mW), which is just 4.8\% off the circuit-level power estimate with PrimeTime.
%while leakage power is 0.115mW for the tile. 
%Active energy of LD\_WT (loading of weights) which occurs only once during initialization, and ACC (accumulation across a subcore) is higher as these operations take 131 cycles while the others take a cycle. 
Active power is estimated by multiplying the synthesized active energy numbers per atomic operation (Table~\ref{table:energy}) with the count of each atomic operation obtained from our functional simulator and dividing the sum by running time.
 For multi-chip applications (CIFAR-10 CNN and ResNet), we assume 4.4pJ/bit for inter-chip I/O, based on state-of-the-art 56Gbps serial link on 28nm (same process as Shenjing)~\cite{shibasaki20163}. %We used their 4.4pJ/bit measurement as our cost of inter-chip I/O communication. 


MNIST MLP is estimated at 120KHz frequency for validation of our architectural power estimates against RTL power numbers. Our functional simulator estimated total power for this network to be at 1.35mW, which is close to the detailed RTL-based power estimate of  1.26mW. The other models are simulated at different frequencies, targeting 30fps throughput.

==> background.tex <==

\begin{comment}

\subsection{Conventional artificial neural networks}
We shall now give a brief introduction into ANNs and their common layer structures. An artificial neuron $i$ will perform weighted sum across all its inputs and apply an activation function to produce the output to the next layer:
\[
y_i=f(\Sigma_{j=1}^n (x_j\cdot w_{j,i})).
\]

{\bf Fully Connected Layer.}
In a fully connected layer~\cite{taylor1996neural}, each neuron receives all inputs from the previous layer to produce the output.

{\bf Convolution Layer.}
In a convolution layer~\cite{lecun1995convolutional}, a kernel sweeps over the input spatial dimensions and perform the weighted sum to produce the output.

{\bf Pooling Layer.}
The pooling layer is a sub-sampling layer that reduces the size of the inputs by taking average, max, etc. operations among the inputs in a kernel.

{\bf Residual Network.}
As the state-of-the-art network structure in deep neural networks, residual networks~\cite{he2016deep} allows a layer's output to be duplicated, with one set going on the usual route, and the other rerouted and added directly to a much later layer.
\end{comment}

\subsection{Spiking neural networks}
SNNs~\cite{maass1997networks} are considered third-generation neural networks. Comparing to ANNs, where the inputs and outputs are real values, SNNs work with input/output of streams of binary values along the time dimension called {\em spike trains}. In this work, we use the integrate-and-fire (IF) model. For each neuron, there are two major steps in the IF model:
\begin{enumerate}
\item {\bf Integration.} The {\em membrane voltage} of the $i$-th neuron at $t$-th time step is the integration of the weighted sum of its binary inputs $b_j(t)$ at $t$ and its value at previous time step $(t-1)$.
\begin{equation*}
V_i(t)=V_i(t-1)+\Sigma_{j=1}^{n}(b_j(t)\cdot w_{j,i}).
\label{eq:integrate}
\end{equation*}

\item {\bf Fire.} If the membrane voltage exceeds a preset threshold, $\theta$, the neuron {\em spikes}, i.e., outputs `1', and the membrane voltage is decreased by the threshold. Otherwise, the neuron outputs `0'. In other words,
if $V_i(t) \geq \theta$ then $y_i(t)=1$, and $V_i(t) = V_i(t)-\theta$. Otherwise, $y_i(t)=0$.

\end{enumerate}

SNN uses the similar network structure and feed-forward inference as ANN, such as multilayer perceptron (MLP) and convolutional neural network (CNN). In this paper, we present both MLP and CNN applications.


\subsection{SNN traits} {\bf Peh: Weaving this into intro}
Compared with ANNs, SNNs are more energy efficient. First, data passing through the layers are binary, so the computation of weighted sum is performed by addition instead of multiplication. This reduces computation power and time significantly. Moreover, a SNN will perform an addition only when the input is $1$, whereas ANN performs multiplications on all neurons across all inputs. In practice, the spiking of neurons is usually sparse, thereby substantially reducing the number of additions.

Using binary instead of full precision floating point data brings about a loss in accuracy. This is the main disadvantage of SNN. However, for most applications, the amount of accuracy loss is usually acceptable. As a matter of fact, there are many researchers working on the compression of ANN by reducing the precision of weights, activations or gradients at the cost of accuracy loss~\cite{han2015deep,zhou2016dorefa,courbariaux2016binarized}.

\subsection{From ANNs to SNNs}
\label{sec:need-PS-Noc}
Due to the discontinuity in the formulation of SNN making the functions to be learnt non-differentiable, there is no robust supervised learning algorithm that is analogous to back-propagation for ANN. Instead, a SNN is usually converted from a pre-trained ANN using the same neural network structure, but with the equivalent ANN's continuous activation replaced by {\em spiking rate encoding}~\cite{Diehll2015}. The input is first converted to a {\em spike train} of a pre-defined length $T$ that has the corresponding normalized value as the spiking rate. Weights of each layer are then normalized such that the spiking rate of each layer correctly represents the ANN activation. 
As an example, suppose we have an ANN whose input is a greyscale picture with pixels of value in $[0, 255]$. Since the equivalent SNN can only take binary inputs of spikes (i.e., 0's and 1's), we need to encode the input. So, the input is first normalized to $[0,1]$ by dividing each pixel value by 255. We then generate a random sequence of spikes (the spike train) of length $T$ as follows: for a pixel value $x\in [0,1]$, we will randomly generate a sequence of about $xT$ ones and $(1-x)T$ zeros. For instance, a black pixel which is 255 will be converted into a $T$-bit spike train of all ones. This spike train is then fed to the neurons in input layer, one spike at a time, across $T$ time steps. Next, for each layer we use the trained ANN weight normalized by the maximum of activation values to ensure that each neuron spikes at most once in a time step. At the output layer, the neuron with the highest number of spikes in $T$ steps is taken as the prediction. 
It has been shown that such a conversion will result in a small accuracy loss~\cite{rueckauer2016theory}. %For not too large networks, the relative loss in this loss is typically less than 5\%. 
In Table~\ref{table:benchmark}, the ``abstract SNN accuracy'' shows the accuracy of our applications converted from ANN to SNN, before mapping onto hardware architectures. Accuracy degrades just 3-6\%.
{\bf Peh: Mentioning key point above in intro to argue that accuracy of SNN models is ok -- need one more huge network}

\begin{comment}
{\bf Peh: Can you add a table showing various ANN network models and their resulting SNN network model accuracy, when everything is run in *software*, regardless of hardware core constraints? Showing that the accuracy loss is very small? So that later we can also highlight how Table 6's Shenjing's accuracy is the same as the SNN software model accuracy. I think we also need a figure or example walking through how this ANN to SNN model conversion is done, or at least how you manually did it for the various models we used in this paper.}
\end{comment}



\subsection{\color{red}Overcoming the partial sum problem}
\label{sec:SNN-to-hw}
{\bf Peh: I think this should be weaved into Architecture of PS NoCs explaining how configurable PS NoCs help with accuracy too, in addition to energy and configuration.}
There is however a second source of accuracy loss. Existing SNN hardware such as TrueNorth~\cite{truenorth} are organized into cores due to hardware constraints as well as for better utilization. Each core computes the weighted sum addition of neurons followed by spike generation.
 Cores communicate strictly using spikes. This presents an issue when layers are too big to fit onto a single core and has to be split. {\color{red} {\em spike}() is a binary function that returns a `1' if its argument exceeds a threshold and `0' otherwise. It is applied to the sum of weights. If we break the sum of (signed) weights into partial sums, i.e. $W = W_1 + \cdots + W_n$, then, as far as we know, there is no function, $\odot$, that will guarantee that
 $spike(W) = spike(W_0) \odot \cdots \odot spike(W_n)$. Systems like TrueNorth
introduce a new layer to combine the spikes from the split layers. 
However, the information loss causes further accuracy loss because depending on the values of the activated weights cancels out each other, spurious spike may sometimes be generated, and this cannot be eliminated entirely by learning in the new layer.} 
\begin{comment}
Consider this simplified extreme: suppose we have a sequence of positive and negative numbers (weights) to be summed. Now suppose that the numbers cancel out and the sum is zero - hence no spike. If we split this into two separate sums, it could be that we ended up with the positive numbers all end up in one sum, and the negative in the other. The net result is that in one core, a spurious spike would be triggered and propagated to the combination layer.
\end{comment}
 
{\color{red}Shenjing eliminates such accuracy loss with its partial sum NoC, which receives the weighted sum of the cores and adds them up precisely. In the above example, Shenjing can produce the total weighted sum over all 784 inputs and produce spikes based on the total sun. This also removes the need for the new combining layer.}

To see the impact of splitting up a layer, we tested a brute-force implementation~\cite{lee2019system} of the MNIST-MLP application (see Table~\ref{table:applications}) for a TrueNorth-like architecture (with no partial sum NoC). %The results are shown in Table~\ref{table:applications}. 
According to their algorithm, in the first layer, when the MNIST input size 784 is larger than a 256-neuron core size, the inputs are split onto 4 cores, and as the layer output size is 512, we need two groups of them with duplicated input. In each group, a core receives 196 input spikes, performs the weighted sum, and spikes with 1/4 of the original threshold. The spikes from 4 cores are then merged by 2 additional cores to produce the final output of the layer. The same method is applied to the second layer. In the end, the method uses 5 additional cores to merge spikes. With 256-neuron cores, we saw MNIST-MLP's accuracy drop from 96.11\% in Table~\ref{table:benchmark} to 93.61\%. The more splits (due to larger models that have to straddle multiple hardware cores), the higher the accuracy loss. To illustrate this, we use the same splitting approach above to map MNIST-MLP onto a range of core sizes. As core size reduces to 128 and 64, thus forcing more splits, we saw the accuracy dropping further to 92.69\% and 88.09\%, respectively. On the other hand, Shenjing maintains the original 96.11\% accuracy of the abstract SNN model.




==> discussion.tex <==
{\bf Core reuse.}
%As CNNs grow deeper, one can always find a network exceeding the hardware limit if all layers are flattened on the cores. Therefore, it is important for a neuromorphic hardware to support core reusing, meaning one hardware core can be used as multiple logic cores. 
Shenjing can easily support a type of core reuse without reloading the weights. In our current mapping of a convolution layer, the input channels are mapped to multiple cores. All channels use identical weights and operations along the spatial dimensions and add up their weighted sums. So, we can use just one core to process all input channels and add them up within the core. The hardware needs to support accumulation of multiple weighted sums from the neuron core, but that cost is small. A more general core reuse strategy where the weights are swapped out and reloaded will have a much higher overhead.

%In principle, core reuse transfers the cost in area to time, thus impacting throughput. For embedded and real-time systems that neuromorphic hardware targets, trading off throughput for area is an important design decision.
%Throughput is important for neuromorphic hardware because they target embedded and real-time systems. Therefore, whether to support core reuse, and what level should the reuse be at is a design choice for architecture developers.

{\bf Mapping optimization.} We used a simple greedy mapping algorithm for our current workflow. This mapping is essentially the well-studied static task graph mapping on multiprocessor problem~\cite{mapping}. We will consider using other more refined algorithms in our future work.

%{\bf Weight Precision.}
%\label{sec:discuss-precision}

%{\bf NoC topology.}
%We chose simple meshes for all our NoCs for several reasons: It provides a universal fabric for software configuration, easing mapping. A lower degree topology like rings will lead to lower power overheads, but heavily constrain the software mapping tool. As our NoCs rely on software for routing and flow control, hardware cost is low anyway. 
%As for hierarchical or clustered topologies, ANNs connections tend to be between layers of many neurons, so there is little locality within a layer that a clustered topology can benefit from. Besides, SNNs are not latency sensitive, so the high average hop count of meshes when compared to hierarchical topologies has little effect on benchmark performance. %{\bf Peh: True and demonstrated in Section 6? If instead of a mesh you have say 16 tiles connected to one router, so fatter routers but fewer hops, will that help?}. 
%Meshes also lend themselves readily to hardware floorplanning and full-chip place-and-route, simplifying fabrication.

%{\bf Multiple chips.}
%Number of IOs across chip, bandwidth, our fully distributed architecture inherently lends itself to multichip.
%Cite current pin bandwidth, serial IO bandwidth to back our assumptions in Section 7 results.
%Peh: I think the above will already be mentioned in results

%{\bf SRAMs with synthesized accumulators for memories.} State-of-the-art neuromorphic architectures have started using non-volatile memory for better energy efficiency~\cite{Jo2010Memristor}~\cite{Ambrogio2016RRAM}~\cite{Wang20152T1R}. For instance, resistive switching memory (RRAM) device has advantages of density, parallel synaptic operations, etc. However, RRAM is still an immature technology that needs much improvement to enable multilevel operation, high on/off ratio, and linear change of the resistance~\cite{Daniele2018NVM}. Shenjing's architecture is orthogonal to the memory technology; we utilize memory compiled SRAMs on the 28nm commercial process, designing the rest of Shenjing around that. The accumulators within our neuron core are synthesized logic, leading to 128 13-bit adders synthesized for each sub core, and (128*4+256=768) 13-bit adders. This is why our neuron core (SRAM+accumulators) takes up 97.6\% of total Shenjing power for the MNIST MLP application. This can be optimized by custom designing in-memory compute SRAMS, like TrueNorth, similar to~\cite{VermaJSSC2017}, which will dramatically reduce the neuron core power and energy. 
% and can be readily optimized just by scaling down the supply voltage. In addition, low power SRAM techniques such as ~\cite{Clinton2017SRAM}~\cite{Guo2018SRAM}~\cite{Chang2017SRAM} can deliver substantial power and energy savings. 

{
%\color{red}
{\bf Optimization of neural network models.}
In ANN, many optimization techniques have been proposed. Some of these such as pruning connections~\cite{han2015deep}, and quantization to weight and gradient~\cite{zhou2016dorefa} are compatible with SNN models, and thus with Shenjing. However, as the activation of SNN is binary, there is little room for further compression. Binarized Neural Network (BNN)~\cite{courbariaux2016binarized} can be considered as a special case of SNN, and Shenjing can support BNN with minimal modification. \cite{ji2018bridge} proposed a compiler to map SNN to hardware architectures by first allocating the network to cores before tuning the weights. Their core allocation algorithms can be used on Shenjing, but the need for weight tuning is eliminated with Shenjing's partial-sum NoCs.

}


{
\color{red}
{\bf Scalability of Shenjing}
SNNs target resource constrained user-cases. Most state-of-the-art SNN accelerators~\cite{Esser11441, spinnaker, inxs} including TrueNorth limit their applications to $32\times 32$ RGB images like Cifar-10, and their models to convolutional networks. Shenjing has a similar target, and we have demonstrated its applications with up to 5863 cores. Thanks to its NoC, it is also the first SNN architecture to support ResNet.}

